On the fractal nature of the partition function $p(n)$ and the divisor functions $d_i(n)$

The partitions of the integers can be expressed exactly in an iterative and closed-form expression. This equation is derived from distributing the partitions of a number in a network that locates each partition in a unique and orderly position. From this representation an iterative equation for the function of the number of divisors was derivated. Also, the number of divisors of a integer can be found from a new function called the trace of the number n, trace(n). As a final preliminary result, using the Bressoud-Subbarao theorem, we obtain a new iterative representation of the sum of divisor function. Using this theorem it is possible to derive an iterative equation for any divisor function and all their networks representation will exhibits a self-similarity behavior. We must then conclude that the intricate nature of the divisor functions results from the fractal nature of the partition function described in the present work.

==> EnEspa__olParticiones <==
REsumen
Las particiones de los números enteros puede expresarse en una ecuación iterativa de manera exacta. Esta ecuación se deduce a partir de distribuir las particiones de un número en una red que ubica a cada particion de manera única. A partir de esta representación en red de las particiones es posible deducir un ecuación iterativa para la función del número de divisores. El número de divisores de un número n puede encontrarse graficamente desde operaciones elementales de suma y resta a partir de la traza del número n, traza(n). 




Se denomina partición p(n) de un numero natural n al numero de formas en las que n puede escribirse como un sumando de numeros naturales sin tomar en cuenta el orden. Por ejemplo, las particiones de 7 son 7, 6+1, 5+1+1, 4+1+1+1, 3+1+1+1+1, 2+1+1+1+1+1, 1+1+1+1+1+1+1, 5+2, 4+1+2, 3+1+1+2, 2+1+1+1+2, 3+2+2, 2+1+2+2, 4+3, 3+1+3. Como existen 15 formas de expresar 7, entoces la p(7) es 15. La pregunta que surge es si existe una forma de expresar en un orden unico cada representación de una partición.

El presente apartado es para determinar una metodología que permita escribir todas las particiones de un numero sin repeticiones y cuya posición sea unica dentro de cada representacion. Para lograr cumplir esta tarea sera muy importante que la metodología seguida establezca en su aplicación un orden en una determinada particion, es decir, que una particion solo podra aparecer de una unica forma.  Iniciaremos esta tarea definiendo algunos conceptos importantates que llamaremos saltos. Cuando nos refiramos a una partición en general nos referiremos a la partición de un mismo número n. 

Definición. Se llaman términos de una partición a cada uno de los sumando que forman una partición de un determinado numero. Estos términos se plasman en un orden determinado. 
Ejemplo
8 5 6 es la particion del numero 19 y 8 es el primer término, 5 el segundo término y 6 el tercer y ultimo término.


Definicion. Se llama un salto de orden 1 a una trasnformación de una particion que brinda otra particion y que consiste en tomar su primer término a y  particionarlo en (a-1) y 1. Este salto tiene como requisito que el término a-1 formado no sea menor que el último término de la partición. 
Ejempo
5 1 3 -> 4 1 1 3
8 5 -> 7 1 5

Definición. Se llama un salto de orden r a una trasnformación de una partición que brinda otra partición y consiste en tomar su primer término a y particionarlo en (a-r) y r. Este salto tiene como requisito que el término a-r formado no sea menor que el último digito de la partición y que el término r no sea mayor que el último termino.
Ejemplo
r = 3
10 4 - > 7 3 4 
r = 5
15 6 -> 10 5 6
Se deduce de esta definición que si una partición inicia con un solo termino n, y se realiza un primer salto de orden r. Todos los saltos que podrian aplicarse a este nueva particion solo podrian tener como orden r o un orden menor que r. 

Definición. Una sucesión no ascendente de saltos ordenada  es aquella en la que a una partición se le aplican sucesivamente saltos cuyos ordenes pueden mantenerse constantes o decender en una o variadas unidades pero nunca ascender. Iniciemos por ejemplo con la partición 7 y apliquemos un salto inicial de orden 1. Entoces la sucesión no ascendente de saltos ordenada de 7 seria: 7 -> 6 1 -> 5 1 1 -> 4 1 1 1 -> 3 1 1 1 1 -> 2 1 1 1 1 1 -> 1 1 1 1 1 1 1, todos los saltos de orden 1. Sin embargo, si iniciamos con un salto de orden dos , la sucesión no ascendente que encontremos seria:
7 -> 5 2 -> 3 2 2 , todos saltos de orden 2, y si ademas hacemosa saltos de orden 1, tendriamos los saltos 5 2 -> 4 1 2 -> 3 1 1 2 - > 2 1 1 1 2, y 3 2 2 -> 3 1 2 2  , todos ellos saltos de orden 1. Podemos ordenar esta sucesión no ascendente de saltos del siguiente modo:
7

52
4 1 2
3 1 1 2
2 1 1 1 2

3 2 2
3 1 2 2
Teorema. Si una partición a1 a2 a3 a4 ... am es el resultado de una sucesión no ascedente de saltos partiendo de un número determinado n , la sucesion a2 a3 a4 ... am a1 es una sucesión de terminos no descendente.

Prueba. Como pueden notarse de la forma en que se van generando los terminos de una sucesión, el termino am es el orden del primer salto, el termino anterior am-1 solo puede ser del orden de am o menor, por lo cual el termino am-1 es igual a am o menor. Similar razonamiento nos lleva a deducir que la sucesión a2 a3 a4 ... am es una sucesión de terminos no descedente. Como por regla general de los saltos, en cada salto el primer término nunca puede ser menor que el ultimo termino, entoces la sucesión a2 a3 a4 ... am a1 forma una sucesión de terminos no descendentes. 

Definición. una sucesión no ascendente de saltos ordenada y completa es aquella en la que a un número n se le aplican todas las sucesiones de saltos ordenadas posibles. Por ejemplo, para el caso del 7 tenemos las siguientes sucesiones ordenadas completas posibles. 
7
#Salto inicial de orden 1
6 1
5 1 1 
4 1 1 1
3 1 1 1 1
2 1 1 1 1 1
1 1 1 1 1 1 1

#Salto inicial de orden 2
5 2
4 1 2
3 1 1 2
2 1 1 1 2

3 2 2 
2 1 2 2

#Salto inicial de orden 3
4 3
3 1 3

Teorema. Los elementos de una sucesión no ascendente de saltos ordenada y completa que parte del numero n constituyen todas las partición del numero n.

Prueba. Para realizar la prueba pasaremos a demostrar primero la unicidad de representación de una partición, lo que involucra demostrar que dos representaciones de una partición cuyos terminos solo se han cambiado de orden no pueden estar presente en una sucesión no ascendente de saltos ordenada. Probaremos tambien que no puede existir particiones con la misma representación. Esto nos permite decir que cada representación es unica y ocupa una posición determinada dentro de esta sucesión. Finalmente probaremos que dada una representación cualequiera, podemos ubicarla inequivocamente dentro de una sucesión no ascendente de saltos ordenada y completa.

En el caso de tener dos representaciones de una particion con unicamente los elementos intercambiados, el segundo elemento debe ser el mismo en ambas representaciones ya que debe ser el menor elemento de todos los elementos presentes. El tercer elemento si existe debe tambien ser el mismo en ambos casos. Pr ejemplo, si este tercer elemento es u en una representación y v en la otra. Si u es mayor que v en la primera representacion, v ya no volveria a aparecer en esta representación a menos que sea igual a u. Ya que v necesariamente debe aparecer en esta representación, v solo podria aparecer si v es igual a u, lo cuales contradictorio. Con el mismo razonamiento se deduce que todos los elementos hasta llegar al penultimo elemento son iguales y ocupan el mismo orden. En el caso del ultimo termino, si en una de las representaciones este es q y en la otra es r, el primer elemento de esta primera representacion seria r, y vise versa, el primer elemento de la segunda representacion seria q. Si q y r son diferentes, en alguna de las representaciones el primer elemento sera menor que el ultimo, en contradicción con las reglas de construcción de las particiones, lo cual, q y r deben ser los mismos en ambas representaciones. De ese modo queda demostrado que existe una unica representacion para cada particion que se encuentre. 

Probaremos a continuación que no pueden aparecer la misma particion dos veces. Para probarlo solo debemos probar que la ruta que produce una particion es unica. Para eso probaremos que el antecesor de una particion es unico. El termino intermedio diferente de 1 más cercano a la izquierda nos informa de salto ha provenido, por ejemplo, si esta particion es de la forma ``a 1 1 ... 1 ... b ... b c ... c ...'' el orden del ultimo salto realizado es 1. Retroceder en este salto nos da la partición antecesora ``a 1 1 ... 1 ... b ... b c ... c ...'' que será el mismo antecesor en ambos casos. Si k es el numero de 1's presentes, las dos particiones consideradas deberian tener como antecesor a   ``(a+kb) b ... b c ... c ...''. Puede deducirse que cada particion solo puede ocurrir de una unica manera, es decir siguiendo una unica ruta. Eso nos demuestra que una particion cualesquiera puede ubicarse inequivocamente dentro de una sucesión no ascendente de saltos ordenada y completa. 

A continuación probaremos que toda particion de un numero n esta contenida dentro de una sucesión no ascendente de saltos ordenada. Para probar ello solo debemos probar que dada una particion podemos llegar al numero n mediante inversa de los saltos de un orden determinado. Debemos iniciar ordenando la particion no ordenada colocando los terminos en orden no descendente. Luego de ello, el último termino de este ordenamiento seria el primer elemento de la representacion que estamos usando en el presente trabajo ``a 1 1 ... 1 ... b ... b c ... c ...''. Esta representacion es unica para cualquier partición del numero n ya que los terminos guardan un orden no descendente desde el término segundo hasta el termino final y primero.Como hemos visto en el parrafo anterior, una particion del tipo ``a 1 1 ... 1 ... b ... b c ... c ...'' puede tener como antecesor último al número (a+kb+lc+md ... ) donde n = a + kl + lc + md. Por lo tanto, sea cual sea la partición no ordenada, podemos ordenarla de modo no descedente como se ha mencionado y podemos ubicarla inequivocamente dentro de la sucesión no ascendente de saltos ordenada y completa. Este caracter de completa es exigido ya que debemos de tomar todos los saltos posibles. Por lo anterior mencionado queda demostrado que los elementos de una sucesión no ascedente de saltos contiene todas las posibles particiones de un determinado número. 


Representación grafica de una partición
En la presente sección detallaremos una forma de representación gráfica de una sucesión no ascendente de saltos ordenada y completa. Como puede notarse de la definición y ejemplos mostrados en la definición de este tipo de sucesión, no se trata de una sucesión lineal sino que indudablemente es una representación ramificada. En la Figura 1 mostramos una posible representación de las particiones del número 15. Puede notarse que con esta representación todos los posibles saltos ordenados no descendentes han sido mostradas. Las lineas verdes en la Figura tiene indicado el orden del salto realizado. Estos primeros saltos van desde un orden 1 hasta un orden 7. Tras cada salto puede uno hacer saltos de un orden igual o menor al salto del orden que le ha precedido. En aquellos grupos de saltos que han inciado con un salto de orden mayor a dos ya no se han colocado la indicación de los saltos de orden 1, pero se los ha agrupado en función del salto de orden dos del cual provienen. Siguiendo este criterio, el grupo de particiones que estan alineadas verticalemente previenen de sucesivos saltos de orden dos. 

Figura1 

Con el objetivo de delucidar la relacion numérica subyacente dentro de esta red, lo que haremos a continuación es remplazar los bloques que surgen de saltos de orden 1 luego de los saltos iniciales por el número de particiones que estos contienen. Esta transformación es mostrada en la Figura 2. Podemos notar en esta figura que verticalmente ocurren progresiones descendentes de razon 2 tras cada salto. Estas progresiones son completas, es decir llegan hasta 2 o 1. Será posible que esto sea una regla?. En el siguiente Teorema demostramos que efectivamente esta es una regla.

Figura 2
Definición. Denominaremos un grupo de particiones de salto de orden 1 al grupo de particiones que parten de una partición que no tiene entre sus terminos el número 1 y que surgen con la sola aplicación continua de saltos de orden 1, incluyendo la particion original . Asi por ejemplo, un grupo de salto de orden 1 que parte de la particion 10 4 seria:
10 4
9 1 4 
8 1 1 4 
7 1 1 1 4
6 1 1 1 1 4
5 1 1 1 1 1 4
4 1 1 1 1 1 1 4
El número de elementos de este grupo de particiones de salto de orden 1 seria 7.

Corolario.El número de saltos posibles de cualquier partición que empieza con el término a y termina con el término m (``a b c ... m'' ) es a-m. Si incluimos la particion orginal entoces el número de elementos de un grupo de particiones de saltos de orden 1 es a-m+1. 
Prueba.En efecto, todo salto de orden 1 disminuye en 1 el primer término y adiciona como segundo término el número 1. Este tipo de saltos solo se puede hacer hasta que este primer término sea igual al primer término m, por lo tanto, el número de saltos de orden 1 de una partición del tipo ``a b c ... m'' sería a-m. Se deduce entoces que el número de elementos de un grupo de particiones de salto de orden 1 seria igual a a-m+1.

Corolario. Si se realiza un salto de orden r>1 desde una partición ``a b c ... m'' hasta una partición ``a-r r b c ...'', el número de elementos del grupo de particiones de salto de orden 1 de la particion ``a-r r b c ... m'' disminuye en r respecto al número de elemento del grupo de particiones de salto de orden 1 de la partición original ``a b c ...''.
Pruba. Ya que la partición resultante del salto de orden r es ``a-r r b c ... m'', el número de elementos del grupo de particiones de saltos de orden 1 que surgen de esta partición es a-r+m+1. Este número es menor en r respecto al número de elementos del grupo de particiones de saltos de orden 1 que surgen de la partición original, a+m-1.

Teorema principal. 

Prueba. Podemos notar que en cuando se realiza un primer salto de orden r, el números de elementos del conjunto de salto de orden 1 de la partición resultante es n-1-2(r-1). En efecto, si se parte del número n, la partición resultante de un salto de orden r es n-r r, el número de elementos del conjunto de saltos de orden 1 de esta partición es n-r-r+1, es decir, n-1-2(r-1). Tras estos primeros saltos es posible realizar todos los saltos no ascendentes y ordenados posibles y como se ha demostrado en los anteriores corolarios, tras un salto de orden s, el número de elementos del conjunto de salto de orden 1 al que pertenece la partición resultante disminuye en s respecto a la partición que lo origino. Entoces se deduce que el número de elementos o particiones de los conjuntos de salto 1 resultantes del primer salto siguen la siguiente formula iterativa peculiar. 

Esta formula iterativa nos permite mapear todos los saltos ordenados no ascedentes desde las particiones originales. Si combinamos este resultado con el anterior resultado para los primeros saltos, llegaremos a la formula.




Función Divisor
----------------
Bing ha establecido un importante téorema que usaremos a continuación y que relaciona nuestro trabajo anterior sobre particiones con la función del número de divisores. Bing y colaboradores establecen primero la definición de una partición con terminos desiguales como aquella partición que tiene todos sus términos diferentes, por ejemplo, la partición de 7 igual a 4 + 2 + 1 es una partición con términos desiguales. Una definición que tambien usa Bing es la de particiones pares o impares , que se definen como las particiones cuyo número de términos es par o impar. Bing define una particion desigual impar o par como aquella particion que tiene todos sus terminos desiguales y que ademas su número de términos es impar o par, respectivamente.

Theorem.ps(n) =d(n) for all positive natural numbers n. (Bng et al.)
donde ps(n) denotes the sum of the smallest numbers of odd partitions of n minus the smallest numbers of even partitions of n, and d(n) denotes the number of divisors of n. 


A continuación construiremos una sucesión  de saltos especial diferente a las sucesiones de saltos anteriores que hemos trabajado en la sección sobre particiones. 


Definición. Se denomina salto de termino inicial invariante "a" y de orden r a  la transformación de una partición de terminos desiguales del tipo a1 a2 ... am en una partición de terminos desiguales resultante de la forma a1 r a2 ... am, con la condición de que r sea menor que cualquier término de la partición y que "a1" no sea igual o menor que el último término am.Este tipo salto convierte una partición de un número n en la partición de un número n+r.

Definición. Se denomina sucesión de saltos descendentes de término inicial invariante a y de terminos desiguales, al conjunto de saltos de termino inicial invariante "a" y cuyos ordenes siguen una sucesion descendente.

Asi por ejemplo, si partimos del número 4. La sucesión de saltos de descendentes de termino inicial invariante 4 y de términos desiguales que inicia con un salto invariante de orden 3 y sigue con los saltos invariantes de orden 2 y 1 es:
4
4 3
4 2 3
4 1 2 3



Definición. Se denomina conjunto completo de saltos descendentes de termino inicial invariante a y de terminos desiguales al conjunto de todas las sucesiones posibles de saltos descedentes de termino inicial invariante a y de terminos desiguales.

Asi por ejemplo, el conjunto completo de saltos descendentes de término incial invariante 4 y de términos desiguales es:

4
4 1

4 2
4 1 2

4 3
4 1 3
4 2 3
4 1 2 3

En otro ejemplo, el conjunto completo de saltos descendentes de término inicial invariante 5 y de términos desiguales es:
5
5 1

5 2
5 1 2

5 3 
5 1 3
5 2 3
5 1 2 3

5 4 
5 1 4
5 2 4
5 1 2 4
5 3 4
5 1 3 4
5 2 3 4
5 1 2 3 4



Lema. Toda particiones de terminos desiguales de un número n esta contenida en unicamente un conjunto completo de saltos descendentes de término incial invariante a1 y de términos desiguales, donde a1 = 1, ..., n.

Prueba. n esta incluida en el conjunto completo de saltos descedentes de termino inicial invariante n. Cualquier otra particion de n de términos desiguales puede ser ordenada en una sucesión descedente tal como a2 a3 ... am a1. Si colocamos el último termino como primer término se tiene la representación de esta partición en la forma siguiente a1 a2 a3 ... am. El número a1 será mayor que todos los otros términos de esta partición ademas a1 es menor que n. Vamos a demostrar que esta particion a1 a2 a3 ... am esta contenida en el conjunto de saltos descendentes de término inicial invariante a1 y de términos desiguales. En efecto, los términos a2, a3, ..., am nos indican que esta partición proviene de la aplicación sucesiva de los saltos invariantes en a1 de orden am, ..., a3 y a2. Siento estos ordenes todos difererentes ya que la particion que estamos considerando tiene todos sus términos diferentes.  Por lo tanto, esta particion estará dentro del conjunto  de saltos descendentes de término inicial invariante a1 y de términos desiguales. 



Es posible representar un conjunto completo de saltos descendentes de término incial invariante a1 y de términos desiguales de una forma grafica como se muestra en la Figura. En esta representación, el orden de los saltos estan marcados con un numero en gris. En verde se ha indicado aquellos saltos que van a generar una partición cuyo número de términos es par, mientras que en marron, aquellos saltos que van a originar particiones cuyo número de términos es impar. 


Corolario
Las particiones del número n cuyos términos son todos diferentes son aquellas particiones que resultan de una sucesión de saltos descendentes de término inicial invariante $a_1$ y de ordenes sucesivos $a_2,a_3,\cdots,am$ con la condición de que $a_1+a_2+\cdots+a_m = n$ 

Prueba. Este resultado surge del hecho de que toda partición del número n esta contenida dentro de alguno de las particiones que surgen de las sucesiones de saltos cuyo término inicial invariante $a_1$ puede tomar el valor de 1 a n. Entoces existe un valor de $a_1$ tal que la sucesión de ordenes sucesivos de saltos invariantes $a_m,\cdots,a_3,_2$ origina una partición de n, por lo tanto $a_m+\cdots+a_3+ a_2 + a_1 = n$  y entoces $a_m+\cdots+a_3+ a_2 = n - a_1$

Lema. 
El término más pequeño de cualquier partición resultante de una sucesión de saltos descedentes con termino incial invariante es siempre el orden del último salto invariante realizado.

Prueba. Ya que se trata de una sucesión descedente de saltos invariantes, entoces el orden de los saltos sucesivos siguen una sucesión descendente, por lo tanto el orden del último salto es el menor término posible de la partición resultante. 

Con el fin de relacionar esta representación con el téorema de Bing se va a cambiar esta representación por la representación de la Figura , en donde solo se van a colocar los términos más pequeños de cada partición, ademas en aquellas particiones cuyo número de términos es par se ha añadido el signo menos. Esta representación toma la forma de una red que denominaremos red de  número de divisores, denominación que cobrara sentido en el sigiuente Lema. 

Definición. Se denomina red de número de divisores a aquella red cuyos primeros vertices son los terminos invariantes $a_1$. Los siguientes vertices corresponden a los términos más pequeños de las particiones que resultan de una sucesición de saltos descedentes de termino inicial invariante $a_1$.

Definición. Se denomina traza de un número natural n, trace(n), a la suma de los vertices de una red de numero de divisores que sean los términos más pequeños de las particiones de n con términos diferentes. 

Lema. 
La trace(n) es igual al número de divisiores de n:
trace(n) = d(n)
Prueba. 
Este resultado se sigue inmediatamente del Teorema de Bing. En efecto, hemos demostrado anterioremente que toda partición con términos diferentes esta contenida en un conjunto completo de saltos descendentes de término incial invariante $a1$ y de términos desiguales, pudiendo a1 tomar los valores de 1 a n. Asi mismo, cada partición solo puede aparecer una unica vez en este conjunto completo debido a que todos los términos son diferentes. Si adicionamos a ello que en un red de número de divisores se ha remplazado las particiones por sus términos más pequeños y ademas que se adiciona el signo menos en las particiones que tienen un número par, entoces inmediatamente se deduce que la traza del número natural n, como ha sido definida, es igual al número de divisores del número n.

Teorema principal
Sea v* igual a :
An,n-1 An-1,n-2  ... A2,1 1* + An,n-1 An-1,n-2 ... A2,1 2* + ... An,n-1(n-1)* + n* = v*

Then v*[n] = d(n)


Prueba. 
En primer lugar , notamos que la red de divisores es una red fractal en el sentido que una parte de ella se repite para que la red evolucione. Hemos colocado en circulos del mismo color aquellas partes que se repiten. La unica diferencia entre estas partes con el mismo color es el signo de los elementos que lo conforman. Por otro lado, la traza un número determinado n es la suma de todos aquellos números que aparecen en la red de divisores que provienen de las particiones de n. Es muy sencillo ubicarlos ya que llegar a estos números desde el número 1 , ubicado en el inicio de la red, toma n pasos (entendiendose paso como el salto al número adjacente en la red). Asi por ejemplo, la traza(6) = 6 + (-1) + (-2) + 1 = 4 = d(6), la traza(5) = 5 + (-1) + (-2) = 2 = d(2), traza(4) = 4 + (-1) = 3 = d(4), traza(3) = 3 + (-1) = 2, traza(2) = 2, traza(1) = 1. A partir de la Figura , vamos a derivar una Figura más general , la Figura, que relaciona la parte de la red anterior al número n, y la parte de la red que se origina desde el número n. Como se vé en la Figura, estas dos partes son identicas solo diferenciandose en el signo de sus elementos. A la primera parte le llamaremos bloque inicial y la segunda parte bloque final. Definiremos en esta red general el vector E_n*. Este vector se generá sumando los términos de la red en la misma dirección en la que se calcula la traza de cualquier número en la red. Para generar este vector, solo se hace uso de los bloques inicial y final relacionados al número n. Asi por ejemplo:
E_1* = [1]
E_2* = [1  2 -1]
E_3* = [1  2  2 -1 -2  1]
E_4* = [1  2  2  3 -3 -1 -2  1  2 -1 ]
E_5* = [1  2  2  3  2 -2 -4 -1 -1  2  1  2 -1 -2  1]     

En general, cada vector E_n* tiene un tamaño de t(n), siendo t(n) el n-esimo número triangular. Podemos extraer de la Figura, que:
E_n* = [E_(n-1)* 0 ... 0] + [0 ... n ... 0] + [0 ... 0 -E_(n-1)] , donde el el número n en el vector [0 ... n ... 0] ocupa la n-enesima posición.
 
 De esta ecuación deducimos que:
E_n* = A_ (n n-1) E_(n-1)* + nI_n*

Por iteración de esta función llegamos a la ecuación:

 



Borradores:

Definición. Se denomina traza de un conjunto completo de saltos descendentes de témino inicial invariante a y de términos desiguales al conjunto de todas las particiones 
 

Ya que $p_s(n)$ se definie en función de los términos más pequeños de las particiones con términos diferentes, estos estan asociados en nuestra red o representación de una partición con el último salto realizado. En efecto, ya que se trata de saltos ordenados no ascendentes, el último salto realizado debe ser de un orden menor o igual a todos los saltos anteriores. Por otro lado, se se realiza un salto desde una partición con número de términos impares, entoces la partición resultante tendra un número de términos pares. En efecto, si la partición a b ... m tiene q términos, tras realizar un salto de orden r obtendriamos la partición a-r r b ... m de q+1 términos. 

Como nos aseguramos que todos los terminos sean diferentes?. Una forma de asegurarnos de ello es que no solo se permitan saltos cuyos ordenes sean descendentes y nuncan ascendentes, ademas que el primer término nunca alcance al último término.

Definición. Una sucesión descendente de saltos ordenada  es aquella en la que a una partición se le aplican sucesivamente saltos cuyos ordenes descienden en una o variadas unidades pero nunca ascender o mantenerse constante. Por ejemplo, si iniciamos con el núemero 11 y realizamos un primer salto de orden 3 entoces surgen la siguiente sucesión descendente de saltos ordenada:
-Salto de orden 3
11
8 3
-Salto de orden 2 de 8 3
6 2 3
-Salto de orden 1 de 6 2 3
5 1 2 3

Definición. Se llama coeficiente de salto al valor del orden del salto multiplicado por $(-1)^(t+1)$ , donde t es el número de términos de la partición a la que se llega con el salto. 

Teorema. El número de divisores de un número n es igual a la suma de todos los coeficientes de todos los saltos descendentes ordenados posibles.
Prueba. Para demostrar este teormea debemos establecer una relacion entre los coeficientes de salto y el teorema de Bing antes comentado. El teorema de Bing establece que  la suma de los términos más pequeño de las particiones impares de términos diferentes (número de términos impares) de n menos la suma de los términos más pequeños de las particiones pares de términos diferentes (número de términos pares) es igual al número de divisores. Esta definición determina entoces que el número de divisores puede expresarse como:
d(n) = a_1 + a_2 + a_3 + a_4 ... a_q + b_1 + b_2 + b_3 + b_4 ... b_r.
Donde $a_i$ representan el menor término de todas las particiones de terminos diferentes y de número impar y $b_i$ representa el menor término de todas las particiones de terminos diferentes y de número par. Desde aqui podemos establecer una relacion entre los términos $a_i$ y $b_i$ con las particiones que forman todas las sucesiones de saltos descendentes y ordenada. En primer lugar debemos establecer que los elementos de las sucesiones de saltos descendentes siempre dan particiones con términos diferentes. En efecto, si dos términos fueran iguales , significaria que dos saltos tiene el mismo orden, lo cual no es posible en las sucesiones de saltos descendentes. La pregunta es si todas las sucesiones de saltos descendentes posibles cubren todas las particiones posibles de terminos diferentes. La respuesta esto último es sí ya cualquier particion de términos diferentes puede ordenarse en forma ascendente y cambiar el último elemento de este ordenamiento en primer término. De modo que si al ordenar en forma ascendente se tiene la sucesión de términos $c_{1}\; c_{2}\; c_{3}\; \cdots\; a_{m-1}\; a_{m}$ y modificamos esta sucesión para darle una forma de las particiones de la red de particiones que hemos desarrollado toma la forma $c_{m}\; c_{1}\; c_{2}\; c_{3}\; \cdots\; a_{m-1}$. Al ver esta partición podemos decir que proviene de una serie de saltos que inician con un salto de $c_{m-1}$ seguida por los saltos $c_3$, $c_2$ y finalmente $c_1$.


Entoces , toda particion de términos diferentes esta dentro del conjunto de todas las posibles sucesion de saltos descendentes que parten del número n.  Finalmente, ya que cada término $a_i$ o $b_i$ son los últimos términos de las particiones, entoces estos términos son iguales a los coeficientes de los saltos. 

Es posible generar una nueva red, que llamariamos la red primaria de divisores que estará determinada por la cantidad de particiones con términos diferentes originada por el salto de mayor orden posible partiendo del número n. Por ejemplo, si tenemos un número n par, el orden del mayor salto posible para producir particiones de terminos diferentes seria el salto n/2-1 que poduciria la partición n/2+1 n/2-1 ,de esta participon podria surgir un salto adicional de un máximo orden de 1 que produciria la partición n/2 1 n/2-1. Por otro lado, si el número n es impar, el orden del mayor salto posible seria (n-1)/2 y la partición resultante seria la partición (n+1)/2 (n-1)/2. De esta partición ya no podria salir una partición adicional de orden 1 o mayor. En una forma general, el salto de mayor orden posible para brindar una partición de términos diferentes partiendo del número n tendria un orden de n/2 - 3/4 - (-1)^{n} /4. Ya que este es el mayor salto, los saltos de menor orden son posibles y con el siguiente corolario probaremos una relacion entre el orden de este salto y el de los otros saltos. 


Corolario. Si el orden del mayor primer salto posible desde un número n es r entoces tras un primer salto de orden r-k solo se podran realizar una sucesión descendentes cuyos ordenes sumen a lo sumo 2k + ((-1)^n+1)/2 y cada salto sea menor que r-k. Ya que r es n/2 - 3/4 - (-1)^{n} entoces cada salto debe ser menor que n/2 - 3/4 - (-1)^{n} - k. 

Corolario. Sean r-k,s,...,u,v el orden la serie de saltos que se realizan desde el número n, donde r es el mayor primer salto posible desde el número n. Se cumple que :
r-k + s + ... + u + v = 2k + ((-1)^n+1)/2 y ademas r-k>s>...>u>v



==> historial/historial2/codigofuente/agradecimiento.tex <==
\begin{center}
\addcontentsline{toc}{chapter}{Agradecimiento}
\vspace*{1.0\baselineskip}
\bf\fontsize{16}{0}\selectfont
AGRADECIMIENTO\\[1.0 cm]
\end{center}
\fontsize{12}{0}\selectfont
Agradezco a mis padres y familia en general por su fortaleza y paciencia durante mis años de estudiante. Agradezco a mi asesor, el Dr. Gino Picasso, por su guía y consejos para encaminarme en el campo de la investigación. Agradezco al Dr. Yannick de Decker por su invaluable apoyo durante mi estancia en Bélgica para realizar el presente trabajo desarrollado en el CENOlI-ULB. A mis compañeras Ruth Quispe Pilco y Sofia Rodriguez por su motivación en diversas etapas de este proyectpo.

==> historial/historial2/codigofuente/capitulo1.tex <==
\section{Partition of a natural number}
The partition p (n) of a natural number n represent the number of ways in which n can be written as an sum of natural numbers without taking into account the order of the additions. For example, the partitions of 7 are 7, 6 + 1, 5 + 1 + 1, 4 + 1 + 1 + 1, 3 + 1 + 1 + 1 + 1, 2 + 1 + 1 + 1 + 1 + 1, 1 + 1 + 1 + 1 + 1 + 1 + 1, 5 + 2, 4 + 1 + 2, 3 + 1 + 1 + 2, 2 + 1 + 1 + 1 + 2, 3 + 2 + 2, 2+ 1 + 2 + 2, 4 + 3, 3 + 1 + 3. Since there are 15 ways to express 7, then p (7) is 15. This introduction section is to determine a methodology that allows writing all partitions of a number without repetitions and whose position is unique within each representation. In order to accomplish this task, it will be very important that the methodology followed establishes an order in a certain partition in its application, that is, that a partition can only appear in a single way. We will start this task by defining some important concepts that we will call jumps. When we refer to a partition in general we will refer to the partition of the same number n.\\

\textbf{Definition.} The \textbf{terms of a partition} are called each of the additions that form a partition of a certain number. These terms are written in a specific order.\\
Example:\\
8 5 6 is the partition of the number 19 and 8 is the first term, 5 the second term and 6 the third and last term.\\


\textbf{Definition.}A \textbf{jump of order 1} is called a transformation of a partition that provides another partition and that consists of taking its first term and dividing it into (a-1) and 1. This jump requires that the term a-1 formed is not less than the last term of the partition.\\
Example:\\
5 1 3 $\to$ 4 1 1 3\\
8 5 $\to$ 7 1 5\\

\textbf{Definition.} A \textbf{jump of order r} is called a transformation of a partition that provides another partition and consists of taking its first term a and partitioning it into (a-r) and r. This jump requires that the a-r term formed is not less than the last digit of the partition and that the r term is not greater than the last term.
Example:\\
r = 3\\
10 4 $\to$ 7 3 4\\
r = 5\\
15 6 $\to$ 10 5 6\\
It follows from this definition that if a partition starts with a single term n, and a first jump of order r is performed. All the jumps that could be applied to this new partition could only have an order r or an order less than r.\\

\textbf{Definition.} A \textbf{non-ascending sequence of ordered jumps} is one in which jumps are successively applied to a partition, the orders of which can remain constant or go down by one or more unit but never go up. Let's start for example with partition 7 and apply an initial jump of order 1. Then the non-ascending sequence of ordered jumps of 7 would be: 7 $\to$ 6 1 $\to$ 5 1 1 $\to$ 4 1 1 1 $\to$ 3 1 1 1 1 $\to$ 2 1 1 1 1 1 $\to$ 1 1 1 1 1 1 1, all jumps of order 1. However, if we start with a jump of order two, the non-ascending sequence that we find would be: 7 $\to$ 5 2 $\to$ 3 2 2, all jumps of order 2, and if we also do jumps of order 1  we get 5 2 $\to$ 4 1 2 $\to$ 3 1 1 2 $\to$ 2 1 1 1 2, and 3 2 2 $\to$ 3 1 2 2, all of them jumps of order 1. We can order this non-ascending sequence of jumps as follows:\\
\\
7\\
\\
5 2\\
4 1 2\\
3 1 1 2\\
2 1 1 1 2\\
\\
3 2 2\\
3 1 2 2\\
\textbf{Theorem.} If a partition $a_{1}\; a_{2}\; a_{3}\; a_{4}\; \cdots\;  a_{4}$ is the result of a non-ascending sequence of jumps starting from a given number n, the sequence $a_{2}\; a_{3}\; a_{4}\; \cdots\; a_{m}\; a_{1}$ is a non-descending sequence of terms. \\

\textit{Proof.} As can be seen from the way in which the terms of a sequence are generated, the term $a_{m}$ is the order of the first jump, the previous term $a_{m-1}$ can only be of the order of $a_{m}$ or less, therefore the term $a_{m- 1}$ is equal to $a_{m}$ or less. Similar reasoning leads us to deduce that the sequence $a_{2}\; a_{3}\; a_{4}\; \cdots \; a_{m}$ is a non-descending sequence of terms. As a general rule of jumps, in each jump the first term can never be less than the last term, then the sequence $a_{2}\; a_{3}\; a_{4}\; \cdots\; a_{m}\; a_{1}$ forms a sequence of non-descending terms.$\blacksquare$\\

\textbf{Definition.} \textbf{A complete and ordered non-ascending sequence of jumps} is one in which all possible ordered jumps are applied to a number n. For example, for the case of 7 we have the following possible complete ordered sequences.\\

7\\
\\
Initial jump of order 1\\
6 1\\
5 1 1\\
4 1 1 1\\
3 1 1 1 1\\
2 1 1 1 1 1\\
1 1 1 1 1 1 1\\
\\
Initial jump of order 2\\
5 2\\
4 1 2\\
3 1 1 2\\
2 1 1 1 2\\
\\
3 2 2\\
2 1 2 2\\
\\
Initial jump of order 3\\
4 3\\
3 1 3\\
\\

\textbf{Theorem.}The elements of an ordered and complete non-ascending sequence of jumps starting from the number n constitute all the partitions of the number n.\\

\textit{Proof.} To carry out the test, we will first demonstrate the uniqueness of the representation of a partition, which involves demonstrating that two representations of a partition whose terms have only been changed in order cannot be present in an ordered and complete non-ascending sequence of jumps. We will also prove that there cannot be partitions with the same representation. This allows us to say that each representation is unique and occupies a certain position within this sequence. Finally, we will prove that given any partition of n, we can place it unequivocally within a complete and ordered non-ascending sequence of jumps starting from n.\\

In the case of having two representations of a partition with only the elements exchanged, the second element must be the same in both representations since it must be the smallest element of all the elements present. The third element if it exists must also be the same in both cases. For example, if this third element is u in one representation and v in the other. If u is greater than v in the first representation, v would no longer appear in this representation unless it is equal to u. Since v must necessarily appear in this representation, v could only appear if v equals u, which is contradictory. With the same reasoning it follows that all the elements up to the penultimate element are equal and occupy the same order. In the case of the last term, if in one of the representations this is q and in the other it is r, the first element of this first representation would be r, and vice versa, the first element of the second representation would be q. If q and r are different, in any of the representations the first element will be less than the last, in contradiction with the construction rules of partitions, which, q and r must be the same in both representations. In this way it is shown that there is a single representation for each partition found.\\

We will now prove that the same partition cannot appear twice. To test it, we only have to prove that the path that a partition produces is unique. For that we will prove that the predecessor of a partition is unique. The intermediate term more closest to the left term informs us of the jump it has come from, for example, if this partition is of the form `` a 1 1 ... 1 ... b ... bc ... c. .. '' the order of the last jump made is 1. Going back in this jump gives us the predecessor partition `` a+1 1 ... 1 ... b ... bc ... c ... '' which will be the same predecessor in both cases. If k is the number of 1's present, the two partitions considered should have as their predecessor `` (a + k) b ... b c ... c ... ''. It can be deduced that each partition can only occur in one unique way, that is, following a unique path. This shows us that any partition can be unequivocally located within a complete and ordered non-ascending sequence of jumps.\\

Since if we start the sequence from the number n, any element we get to will be a partition of n. Therefore, the set of elements of the non-ascending sequence of ordered and completed jumps is contained within the elements that make up the partition of the number n. To prove that these two sets are equal, simply prove that that every partition of a number n is contained within a non-ascending sequence of ordered and completed jumps. To prove this, we only have to prove that given a partition we can reach the number n by inverse of the jumps of a certain order. We must start by ordering the unordered partition by placing the terms in non-descending order. After that, the last term of this ordering would be the first element of the representation that we are using in the present work `` a 1 1 ... 1 ... b ... bc ... c ... '' . This representation is unique for any partition of the number n since the terms keep a non-descending order from the second term to the final term and first. As we have seen in the previous paragraph, a partition of the type `` a 1 1 ... 1 ... b ... bc ... c ... '' can have as its last ancestor the number (a + kb + lc + md ...) where n = a + kl + lc + md. Therefore, whatever the unordered partition, we can order it in a non-descending way as mentioned and we can place it unequivocally within the complete and ordered non-ascending sequence of jumps. This character of complete is required since we must take all the possible jumps. For the above mentioned it is shown that the elements of a non-ascending sequence of jumps contains all the possible partitions of a certain number. $\blacksquare$\\

\subsection{Main Theorem} 
In this section we will detail a form of graphical representation of an ordered and complete non-ascending sequence of jumps. As can be seen from the definition and examples shown in the definition of this type of sequence, it is not a linear sequence but will undoubtedly be a branched representation. In Figure \ref{Secuencia} we show a possible representation of the partitions of the number 15. It can be noted that with this representation all possible non-descending ordered jumps have been shown. The green lines in the Figure \ref{Secuencia} show the order of the jump performed. These first jumps go from order 1 to order 7. After each jump one can make jumps of an order equal to or less than the jump of the order that preceded it (brown lines). In those groups of jumps that have started with a jump of order greater than 1, the indication of the jumps of order 1 has no longer been placed, but they have been grouped according to the jump of order two from which they come. Following this criterion, the group of partitions that are vertically aligned come from successive jumps of order two. 
\begin{figure}[!ht]
\centering
\includegraphics[scale=0.50]{figuras/secuencia_3.png}
\caption[]{Layaout of the representation of the integer number 15}
\label{Secuencia}
\end{figure}

In order to elucidate the underlying numerical relationship within this network, what we will do next is to replace the blocks that arise from jumps of order 1 after the initial jumps by the number of partitions they contain. This transformation is shown in Figure \ref{Secuencia_numeros}. We can notice in this figure that descending progressions of ratio 2 occur vertically after each jump. These progressions are complete, that is, they go up to 2 or 1. Could this be a rule? In the following Theorem we show that this is indeed a rule.

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.80]{figuras/secuencia_numbers.png}
\caption[]{Layaout of the número of partitions of the number 15}
\label{Secuencia_numeros}
\end{figure}

\textbf{Definition.} We will name \textbf{jump set of order 1} to the set of partitions that are the result of the continuous application   of order 1 jumps, including the original partition. For example,  a jump set of order 1 starting from partition 10 4 is:\\
10 4\\
9 1 4\\
8 1 1 4\\
7 1 1 1 4\\
6 1 1 1 1 4\\
5 1 1 1 1 1 4\\
4 1 1 1 1 1 1 4\\
The number of elements in this jump set of order 1 is 7.\\

\textbf{Corollary.} The number of possible jumps of any partition that begins with the term a and ends with the term m (`` a b c ... m '') is a-m. If we include the original partition, then the number of elements in a jump set of order 1 is a-m + 1.\\
\textit{Proof.} In fact, each jump of order 1 decreases the first term by 1 and adds the number 1 as the second term. This type of jump can only be performed until this first term is equal to the first term m, therefore, the number of jumps of order 1 of a partition of type `` a b c ... m '' would be a-m. It follows then that the number of elements in a jump set of order 1 is equal to a-m+1.\\

\textbf{Corollary.}If a jump of order r> 1 is made from a partition `` a b c ... m '' to a partition `` a-r r b c ... '', the number of elements in the jump set of order 1 of the the partition `` a-r r b c ... m '' is decremented by r with respect to the number of elements of the jump set of order 1 of the original partition `` a b c ... m ''.\\
\textit{Proof.} Since the partition resulting from the jump of order r is `` a-r r b c ... m '', the number of elements of the jump set of order 1 that arise from this partition is a-r + m + 1. This number is smaller in r with respect to the number of elements of the jump set of order 1 that arise from the original partition, a+m-1.\\

\textbf{Main Theorem.} If n is a natural number and p(n) represent the number of partitions of the number n, then 

\begin{equation}
\centering
p(n) = \sum_{i=0}^{floor(\frac{n}{2})} \mathscr{P}(i,n+1-2i)
\end{equation}
\begin{equation}
\centering
\mathscr{P}(s,t) =  \sum_{i=1}^{ceil(\frac{t}{s})} \mathscr{P}(s-1,t-s(i-1))
\end{equation}
\begin{equation}
\centering
\mathscr{P}(0,t) = 1
\end{equation}

\textit{Proof.} We can notice that when a first jump of order r is performed, the number of elements of the jump set of order 1 of the resulting partition is n-1-2(r-1). Indeed, if we start from the number n, the partition resulting from a jump of order r is n-r r, the number of elements of the set of jumps of order 1 of this partition is n-r-r + 1, that is, n-1-2(r-1). After these first jumps it is possible to perform all possible non-ascending and ordered jumps and as has been shown in the previous corollaries, after a jump of order s, the number of elements of the jump set of order 1 to which the resulting partition belongs decreases. itself with respect to the partition that originated it. Then it follows that the number of elements or partitions of the jump sets 1 resulting from the first jump follow the following peculiar iterative formula.
\begin{equation}
\centering
\mathscr{P}(s,t) =  \sum_{i=1}^{ceil(\frac{t}{s})} \mathscr{P}(s-1,t-s(i-1))
\end{equation}
\begin{equation}
\centering
\mathscr{P}(0,t) = 1
\end{equation}

Where $\mathscr{P}(s,t)$ gives us the number of possible partitions that can arise after having made an initial jump of order s starting from a partition that originates a set of jumps of order 1 whose elements are in total t. . This iterative formula allows us to map all non-ascending ordered jumps from the original partitions. If we combine this result with the previous result for the first jumps, we will arrive at the formula.$\blacksquare$
\begin{equation}
\centering
p(n) = \sum_{i=0}^{floor(\frac{n}{2})} \mathscr{P}(i,n+1-2i)
\end{equation}


==> historial/historial2/codigofuente/capitulo2.tex <==
\section{Divisor fuction d(n)}
If $p_s(n)$ denotes the sum of the smallest numbers of odd partitions of n minus the smallest numbers of even partitions of n, and d(n) denotes the number of divisors of n. For every numbers n, $p_s(n)$ equals d(n). This is a  general relation between the smallest numbers of partitions into unequal parts and the number of divisors and it is a theorem from Bing et al.\cite{bing1995relation}.\\

If we analyze this result based on our previous results, some very important relationships emerge. In the first place, since $ p_s (n) $ is defined in terms of the smallest terms, these are associated in our network or representation of a partition with the last jump made. Indeed, since they are non-ascending ordered jumps, the last jump performed must be of an order less than or equal to all the previous jumps. On the other hand, a jump is made from a partition with an odd number of terms, then the resulting partition will have a number of even terms. Indeed, if the partition `` a b c ... m '' has q terms, after performing a jump of order r we would obtain the partition `` a-r r b c ... m '' of q + 1 terms.\\

\textbf{Definition.} An \textbf{ordered descending sequence of jumps} is one in which jumps are successively applied to a partition whose orders descend by one or more units but never rise or remain constant. For example, if we start with the number 11 and perform a first jump of order 3 then the following descending orderly sequence of jumps appears:\\
Jump of order 3\\
11\\
8 3\\
Jump of order 2 of 8 3\\
6 2 3\\
Jump of order 1 of 6 2 3\\
5 1 2 3\\

\textbf{Definition. }The \textbf{jump coefficient} is the value of the jump order multiplied by $ (-1)^{t + 1} $, where t is the number of terms of the partition reached with the jump.\\

\textbf{Theorem.}The number of divisors of a number n is equal to the sum of the number n and the sum of all coefficients of all possible jumps in all ordered descending sequence of jumps starting from the number n.\\

\textit{Proof. }To prove this theory, we must establish a relationship between the jump coefficients and Bing's theorem discussed above. Bing's theorem states that the sum of the smallest terms of the odd partitions of different terms (number of odd terms) of n minus the sum of the smallest terms of the even partitions of different terms (number of even terms) is equal to the number of divisors. This definition then determines that the number of divisors can be expressed as:
\begin{equation}
\centering
d(n) = a_1 + a_2 + a_3 + a_4 + \cdots+ a_q - b_1 - b_2 - b_3 - b_4 - \cdots - b_r
\end{equation}

Where $a_i$ represents the smallest term of all partitions of different and odd-numbered terms and the $b_i$ represents the smallest term of all partitions of different and even-numbered terms. From here we can establish a relationship between the terms $a_i$ and $b_i$ with the partitions that form all the descending and ordered jump sequences. First of all, we must establish that the elements of descending jump sequences always give partitions with different terms. Indeed, if two terms were equal, it would mean that two jumps have the same order, which is not possible in descending jump sequences. Another question is whether all possible descending jump sequences cover all possible partitions of different terms. The answer to the latter is yes and any partition of different terms can be ordered in ascending order and change the last element of this order first. So if when sorting in ascending order we have the sequence of terms $ c_{1} \; c_2 \; c_3 \; \cdots \; c_{m-1} \; c_{m} $ and we modify this sequence to give it a shape of the partitions of the partition network that we have developed takes the form $ c_ {m} \; c_1 \; c_2 \; c_3 \; \cdots \; c_{m-1} $. When we see this partition we can say that it comes from a series of jumps that start with a jump of order $c_{m-1} $ followed by the jumps of order $c_{m-2}$,$\cdots$, $c_3$, $ c_2 $ and finally a $ c_1 $ order jump. Therefore, every partition of different terms is within the set of all possible descending jumps starting from the number n. Finally, since each term $ a_i $ or $ b_i $ are the last terms of the partitions, then the sum of all these terms are equal to the coefficients of the jumps of all the descending jumps starting from the number n $\blacksquare$.




\section{Miscelaneous}
\subsection{Some representation in a graph of $f^2(n)$}
As shown in Figure \ref{Secuencia}, the terms that arise from a complete jump down are a series of numbers of arirmetic ratio 2, both those that arise from a jump of the first order and those that arise from a jump of the second order. We can represent these numbers with the symbol $f^2(n)$, in which the number two indicates that we are taking a sum following a ratio of order two. For example, $f^2(5) = 5 + 3 + 1$ and $f^2(6) = 6 + 4 + 2$. The reason for this data set to be a descending ratio two series is that each of the first two representations of these series do not have two 1's that would allow them to jump down, therefore, each time the jump is made , the number of representations decreases by two.\\

As shown in Figure, using the function $f^2(n) = \circled{n}= \sum_{i=0}^{} n-2i$ and also the function $f ^ 1 (n) = \squared{n} = n$, we can represent the network in an evolutionary way. 
\begin{figure}[!ht]
\centering
\includegraphics[scale=0.3]{figuras/red.png}
\caption[]{Partition of the integer number 15}
\label{Red}
\end{figure}



In Figure \ref{Red}, we had replaced all the representation in a complete jump down with the function $f^2(n) = \circled{n}$ . The nodes related in a left-jump in this network are nodes that arise from a second order jump up, the nodes related in a right-jump arise from a first order jump. If we add all the terms that appear within this representation we will have the partition of the number 15 (Equation \ref{p15}). As we have previously established, each element of the data sequence is generated in a unique way and occupies a unique position within the network, likewise, this uniqueness also confers a uniqueness to each element of the network representation of this sequence of representations. 
\begin{align*}
\centering 
p(15) &= \squared{15} + \circled{12} + \circled{10} + \circled{7} + \circled{4} + \circled{1} + \circled{8} + \circled{5} + \circled{2} + \circled{4} + \circled{1} + \circled{6} + \\&+ \circled{3} + \circled{2} + \circled{1} + \circled{4} + \circled{1} + \circled{2}\\  p(15) &= 15 + 42 + 30 + 16 + 6+ 1 +20 + 9 + 2+ 6 +1 +12 + 4 + 2 +1 + 6 +1 +2 \\
p(15) &= 176  
\label{p15}
\end{align*}
The Figures \ref{Red20-21-22} and \ref{Red23-24-25} shown the network representation of the partion of the numbers 20,21,22,23,24 and 25. There are notable peculiarities in these representations. We will first point out that there is an initial branch in all distributions that follows the following series $ \squared{n}$,$\circled{n-3}$,$\circled{n-5}$, $\circled{n-7}$,$\circled{n-9}$,$\circled{n-11}$, $\cdots$.\\
\begin{landscape}
\begin{figure}
\centering
\includegraphics[scale=0.36]{figuras/red20-21-22.png}
\caption[]{Network representations of the partition of the integer numbers 20,21 and 22}
\label{Red20-21-22}
\end{figure}
\end{landscape}

\begin{landscape}
\begin{figure}
\centering
\includegraphics[scale=0.32]{figuras/red23-24-25.png}
\caption[]{Network representations of the partition of the integer numbers 23,24 and 25}
\label{Red23-24-25}
\end{figure}
\end{landscape}


\begin{landscape}
\begin{figure}
\centering
\includegraphics[scale=0.8]{figuras/red-abstracto-markoviana.png}
\caption[]{Network representations of the partition of the integer n}
\label{Red-abstract-markovian}
\end{figure}
\end{landscape}


==> historial/historial2/codigofuente/dedicatoria.tex <==
\begin{flushright}
\vspace*{\fill}
\addcontentsline{toc}{chapter}{Dedicatoria}
\vspace*{1.0\baselineskip}
\textbf{\fontsize{16}{0}\selectfont
DEDICATORIA\\[1.0 cm]}

\fontsize{12}{0}\selectfont
A mis padres, mis abuelos, hermanos , sobrinas y cuñada. A Ruth y a todos los jovenes que como ella y yo se adentran en un tema desconocido con ansias de saber y aprender para sacar adelante el pais con amor y paz
%\vspace*{\fill}
\end{flushright}

==> historial/historial2/codigofuente/portada.tex <==
\thispagestyle{empty}
\begin{center}
\textbf{\fontsize{18}{0}\selectfont
UNIVERSIDAD NACIONAL DE INGENIERIA\\[1.0 cm]}

\fontsize{16}{0}\selectfont
FACULTAD DE CIENCIAS\\[1.0 cm]

\includegraphics[scale=0.12]{figuras/logouni.png}\\[1.0cm]

\textbf{\fontsize{16}{0}\selectfont
TESIS\\[0.5 cm]}

\textbf{\fontsize{16}{0}\selectfont
``SIMULACIÓN DE PROCESOS QUÍMICOS : APLICACIÓN DE LAS TERMODNINAMICA FUERA DEL EQUILIBRIO, LA DINAMICA DE MONTECARLO O LA GENERACIÓN DE REDES DE REACCIONES''\\[1.6 cm]}

\fontsize{15}{0}\selectfont
PARA OBTENER EL GRADO ACADÉMICO DE MAESTRO EN CIENCIAS EN QUÍMICA\\[1.0 cm]

\textbf{\fontsize{16}{0}\selectfont
ELABORADA POR :\\[0.5 cm]}

\fontsize{15}{0}\selectfont
ROMULO LENCIO CRUZ SIMBRON\\[1.0 cm]

\textbf{\fontsize{16}{0}\selectfont
ASESOR : \\[0.5 cm]}

\fontsize{15}{0}\selectfont
Dr. GINO ITALO PICASO ESCOBAR\\[1.0 cm]

\textbf{\fontsize{16}{0}\selectfont
LIMA-PERÚ \\[0.5 cm]}

\textbf{\fontsize{16}{0}\selectfont
2020\\[0.5 cm]}

\end{center}




==> historial/historial2/codigofuente/preambulo.tex <==
\usepackage[lmargin=3cm,rmargin=3cm,top=1.5cm,bottom=2cm]{geometry}
\pagestyle{headings}
\usepackage[T1]{fontenc}
\usepackage{times}
\usepackage[utf8]{inputenc}
\usepackage[spanish,es-tabla]{babel}
\parindent = 0cm
\usepackage{amsmath}
\usepackage{amssymb,amsfonts,latexsym,cancel}
\usepackage{array}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage[colorlinks = true, linkcolor = blue, citecolor = blue, urlcolor = blue]{hyperref}
%\usepackage{subfigure}
\usepackage{anyfontsize}
\usepackage[thinc]{esdiff}

\usepackage{booktabs,mathptmx}
\usepackage{upgreek}
\usepackage[version=4]{mhchem}
\usepackage{amsthm,empheq}
\usepackage{mathtools}
\usepackage[thinc]{esdiff}
\usepackage{blkarray}
\usepackage{nccmath}
\usepackage{apacite}
\usepackage{setspace}

%\renewcommand{\baselinestretch}{1.5}
\usepackage{mathrsfs}
\usepackage{bm}

\usepackage{chemfig}
\usepackage{chemscheme} 

\usepackage{chemmacros}
\chemsetup{modules={scheme}}
\DeclareChemTranslation{scheme}{spanish}{esquema} 
\DeclareChemTranslation{Scheme}{spanish}{Esquema}

\usepackage{tikz}
\usetikzlibrary{tikzmark,calc}

\usepackage{float}
\floatstyle{plaintop}
\restylefloat{table}
\usepackage{tabularx}

%Comando para hacer encerrar ecuaciones en circulos
\makeatletter
\newcommand\mathcircled[1]{%
  \mathpalette\@mathcircled{#1}%
}
\newcommand\@mathcircled[2]{%
  \tikz[baseline=(math.base),red] \node[draw,circle,inner sep=0.5pt] (math) {$\m@th#1#2$};%
}
\makeatother
%Comando para hacer encerrar ecuaciones en circulos azules
\makeatletter
\newcommand\mathcircledblue[1]{%
  \mathpalette\@mathcircledblue{#1}%
}
\newcommand\@mathcircledblue[2]{%
  \tikz[baseline=(math.base),blue] \node[draw,circle,inner sep=0.5pt] (math) {$\m@th#1#2$};%
}
\makeatother
%Comando para hacer encerrar ecuaciones en circulos naranja
\makeatletter
\newcommand\mathcirclednaranja[1]{%
  \mathpalette\@mathcirclednaranja{#1}%
}
\newcommand\@mathcirclednaranja[2]{%
  \tikz[baseline=(math.base),orange] \node[draw,circle,inner sep=0.5pt] (math) {$\m@th#1#2$};%
}
\makeatother
%Comando para hacer encerrar ecuaciones en circulos cyan
\makeatletter
\newcommand\mathcircledcyan[1]{%
  \mathpalette\@mathcircledcyan{#1}%
}
\newcommand\@mathcircledcyan[2]{%
  \tikz[baseline=(math.base),cyan] \node[draw,circle,inner sep=0.5pt] (math) {$\m@th#1#2$};%
}
\makeatother
%Comando para hacer encerrar ecuaciones en circulos marron
\makeatletter
\newcommand\mathcircledmarron[1]{%
  \mathpalette\@mathcircledmarron{#1}%
}
\newcommand\@mathcircledmarron[2]{%
  \tikz[baseline=(math.base),brown] \node[draw,circle,inner sep=0.5pt] (math) {$\m@th#1#2$};%
}
\makeatother
%Comando para hacer encerrar ecuaciones en circulos amarillo
\makeatletter
\newcommand\mathcircledamarillo[1]{%
  \mathpalette\@mathcircledamarillo{#1}%
}
\newcommand\@mathcircledamarillo[2]{%
  \tikz[baseline=(math.base),yellow] \node[draw,circle,inner sep=0.5pt] (math) {$\m@th#1#2$};%
}
\makeatother

\usepackage{csquotes}
\usepackage{parskip} % Package to tweak paragraph skipping
\usepackage{authblk}
\usepackage{blindtext}
\usepackage{lscape}
\usepackage{pdflscape}

\usepackage{authblk}
\usepackage{hyperref}

==> historial/historial2/codigofuente/resumen.tex <==
\begin{center}
\addcontentsline{toc}{chapter}{Resumen}
\vspace*{1.0\baselineskip}
\bf\fontsize{16}{0}\selectfont
RESUMEN\\[1.0 cm]
\end{center}
\fontsize{12}{0}\selectfont
En el presente trabajo abordamos tres tipos de problemas en los cuales los procesos de simulacion computacionar seran de utilidad. Abordamos en primer lugar el proceso de simulación de un sistema autocalitico que presenta oscilaciones atenuadas que tiene una gran relevancia en la regulación y trasporte de los oxidos de nitrogeno en los seres vivos. Posteriormente mostraremos nuestros resultados en la simulaciones de procesos de cristalización de aminoacidos y su relaciones con las nuevas teorias de crisalización, especialmente con la teoria de clusters de prenucleación. Finalmente mostraremos los resultados de las simulaciones en redes de reacciones atmosfericas. Estas redes atmosfericas son de gran utilidad considerando la basta cantidad de compuestos desconocidos que juegan un rol importante en los procesos de nuestra aatmosfera o la de otros planetas. \\

Al respecto de nuestra primera parte, Anatoly Vanin y su grupo de investigación han llevado a cabo durante más de 50 años un extenso estudio sobre el papel preponderante que juega los complejos de dinitrosil hierro en los sistemas biológicos y porque estas estructuras simples constituyen una \textit{working form} del óxido nítrico endógeno en los sistemas vivos. La participación del óxido nítrico como un regulador universal, presente en todas las formas de vida conocida le ha llevado a la importante conclusión del papel preponderante, tanto presente como pasado, que han jugado los DNICs en la definición de los procesos metabólicos de los seres vivos. El ion ferroso, los tioles y el óxido nítrico son los bloques fundamentales mediante los cuales una química rica en muchos aspectos sobresale por sobre otros mecanismos de regulación gracias a la capacidad de estabilización y activación que presentan los complejos de hierro dinitrosil. Un aspecto muy interesante para la comunidad que estudia procesos fuera del equilibrio es el trabajo del Dr. Vanin de la reacción entre el ion ferroso y nitrosotioles (Vanin et al., 2004). Dichos sistemas muestras oscilaciones temporales atenuadas de la concentración de DNIC en un intervalo de tiempo de 500 a 2500 s. Así mismo, experimentos realizados sobre una película de nitrosotioles impregnados sobre un soporte de vidrio al que se le deja caer una gota de solución de hierro y tioles presenta estructuras circulares concéntricas de alrededor de 6 mm de diámetro que se van atenuando durante un intervalo de tiempo de 0 a 10 s y se dirigen hacia el centro de origen de la gota (Vanin et al., 2006;Vanin, et al., 2010). En el caso de las oscilaciones atenuadas de la concentración de DNIC, las mismas han sido seguidas por espectroscopia de electron paramagnetic resonance (EPR) debido a la naturaleza paramagnética de DNIC. Ya que un intermedio previo a la aparición de DNIC es MNIC, un mononitrosil hierro de naturaleza paramagnética,  el seguimiento de la reacción de DNIC se ha realizado en concentraciones de hierro y nitrosotioles bajo las cuales la presencia de MNIC se ve restringida a los primeros estadios de la reacción, ello con el objetivo de que la señal de DNIC (factor g=2.03) no se vea afectada por la señal asignada a MNIC (factor g=2.04). El Dr. Vanin señala en su artículo que pueden descartarse un \textit{instrumental artifact }causado por alguna desviación en  las frecuencias de resonancia, sin embargo, señala que ello no ha sido notado debido a  que la posición de la señal de EPR no cambio con respecto a la escala de campo magnético durante el tiempo de adquisición de los datos. Otro sustento que menciona el Dr. Vanin en su artículo es que el modelamiento computacional de un esquema cinético propuesto por él logra presentar oscilaciones en un rango plausible de condiciones iniciales y valores de las constantes cinéticas. Acording to Clarke \cite{clarke1988stoichiometric}.\\

La segunda parte de la presente Tesis aborda el tema de amplificación quiral  mediante procesos de cristalización de aminoacidos. Mediante un modelo de red y usando la dinámica de Monte Carlo, el presente trabajo aborda los procesos de amplificación quiral que llevan a un crecimiento rápido del exceso enantiomérico en solución partiendo de una mezcla racémica o cercana al punto racémico. Se busca comprender el  efecto de variables como la temperatura, la concentración o las constantes que definen las energías de interacción, en la concentración de equilibrio tras su evolución dinámica. La evolución dinámica puede involucrar un camino hacia un equilibrio de fases en un sistema D-L-S, donde D y L representan moléculas quirales opuestas y S representa un solvente poco soluble hacia ellos. También se estudiará la dinámica que lleva a una amplificación quiral  producto de una reacción de autocatálisis asimétrica según el modelo de Frank, o una variante, que logre racionalizar los resultados obtenidos por Kenso Soai. Por último, ambas dinámicas, la del equilibrio de fases y la de la reacción asimétrica, se unirían en un solo modelo que permita estudiar sus correlaciones y sus propiedades emergentes. La presente Tesis ha logrado reproducir de manera cualitativa los resultados obtenidos por Klussman al buscar comprender el equilibrio de fases D-L-S usando aminoácidos. Se ha escrito un código en C++ que logra modelar la evolución dinámica de los mismos partiendo de un arreglo aleatorio hacia un estado de equilibrio de mínima energía potencial. Los resultados permiten obtener diagramas de equilibrio de fases muy similares a los obtenidos experimentalmente.\\

